Negotiation as Concurrency Primitive

This paper introduces negotiations, a model of concurrency close to Petri nets, with multi-party negotiations as concurrency primitive. We study two fundamental analysis problems. The soundness problem consists in deciding if it is always possible for a negotiation to terminate successfully, whatever the current state is. Given a sound negotiation, the summarization problem aims at computing an equivalent one-step negotiation with the same input/output behavior. The soundness and summarization problems can be solved by means of simple algorithms acting on the state space of the negotiation, which however face the well-known state explosion problem. We study alternative algorithms that avoid the construction of the state space. In particular, we define reduction rules that simplify a negotiation while preserving the sound/non-sound character of the negotiation and its summary. In a first result we show that our rules are complete for the class of weakly deterministic acyclic negotiations, meaning that they reduce all sound negotiations in this class, and only them, to equivalent one-step negotiations. This provides algorithms for both the soundness and summarization problems that avoid the construction of the state space. We then study the class of deterministic negotiations. Our second main result shows that the rules are also complete for this class, even if the negotiation contains cycles. Moreover, we present an algorithm that completely reduces all sound deterministic negotiations, and only them, in polynomial time.

==> tikz/shortcut_easy/shortcut_easy2.tex <==
\begin{tikzpicture}
\nego[ports=1,id=n0]{0,0}
\node[right = 0.1cm of n0_P0, font=\large] {$n_0$};
\nego[ports=1,id=n1]{-1,-1.5}
\node[left = 0.1cm of n1_P0, font=\large] {$n_1$};
\nego[ports=1,id=n2]{1,-1.5}
\node[right = 0.1cm of n2_P0, font=\large] {$n_2$};
\nego[ports=1,id=n3]{0,-3}
\node[above = 0.1cm of n3_P0, font=\large] {$n_3$};
\nego[ports=1,id=nf]{0,-4.5}
\node[right = 0.1cm of nf_P0, font=\large] {$n_f$};
\pgfsetarrowsend{latex}
\path (n0_P0)
	edge (n1_P0)
	edge (n2_P0);
\path (n1_P0) edge (n3_P0);
\path (n2_P0)
	 edge (n3_P0)
	 edge (nf_P0);
\path (n3_P0) edge (nf_P0);
\end{tikzpicture}

==> tikz/shortcut_easy/shortcut_easy4.tex <==
\begin{tikzpicture}
\nego[ports=1,id=n0]{0,0}
\node[right = 0.1cm of n0_P0, font=\large] {$n_0$};
\nego[ports=1,id=n1]{-1,-1.5}
\node[left = 0.1cm of n1_P0, font=\large] {$n_1$};
\nego[ports=1,id=n2]{1,-1.5}
\node[right = 0.1cm of n2_P0, font=\large] {$n_2$};
\nego[ports=1,id=n3]{0,-3}
\node[above = 0.1cm of n3_P0, font=\large] {$n_3$};
\nego[ports=1,id=nf]{0,-4.5}
\node[right = 0.1cm of nf_P0, font=\large] {$n_f$};
\pgfsetarrowsend{latex}
\path (n0_P0)
	edge (n1_P0)
	edge (n2_P0);
\path (n1_P0)
	edge (nf_P0);
\path (n2_P0)
	edge (nf_P0);
\path (n3_P0) edge (nf_P0);
\end{tikzpicture}

==> useless.tex <==
\begin{tikzpicture}
\nego[text=pq,id=n0,spacing=1.3]{0,0}
\node[above right = -0.2cm and 0.2cm of n0_P0, font=\large] {$n$};
\nego[text=qp,id=n1,spacing=1.3]{-2.3,-2}
\node[above right = -0.2cm and 0.2cm of n1_P0, font=\large] {$n''$};
\nego[text=pq,id=n2,spacing=1.3]{1,-2}
\node[above right = -0.2cm and 0.2cm of n2_P0, font=\large] {$n'$};
\pgfsetarrowsend{latex}
\draw (n0_P0) -- (0,-1) -- (n1_P1);
\draw (n0_P0) -- (0,-1) -- (n2_P0);
\labelEdge[start=n0_P0,end=n2_P0,dist=0.8,shift={-0.6,0}]{\texttt{r}}
\draw (n0_P1) -- (n2_P1);
\labelEdge[start=n0_P1,end=n2_P1,dist=0.8,shift={-0.4,0}]{\texttt{r}}

\draw[=>] (0.5,-2.5) -- (0.5,-3.5);
\node[anchor=west] at (0.5,-3) {\color{blue}{Useless arc rule}};
\draw (-2.3,-0.5) -- (n1_P0);

\begin{scope}[shift={(0,-4)}]
\pgfsetarrowsend{}
\nego[text=pq,id=n0,spacing=1.3]{0,0}
\node[above right = -0.2cm and 0.2cm of n0_P0, font=\large] {$n$};
\nego[text=qp,id=n1,spacing=1.3]{-2.3,-2}
\node[above right = -0.2cm and 0.2cm of n1_P0, font=\large] {$n''$};
\nego[text=pq,id=n2,spacing=1.3]{1,-2}
\node[above right = -0.2cm and 0.2cm of n2_P0, font=\large] {$n'$};
\pgfsetarrowsend{latex}
\draw (n0_P0) -- (n2_P0);
\labelEdge[start=n0_P0,end=n2_P0,dist=0.8,shift={-0.4,0}]{\texttt{r}}
\draw (n0_P1) -- (n2_P1);
\labelEdge[start=n0_P1,end=n2_P1,dist=0.8,shift={-0.4,0}]{\texttt{r}}
\draw (-2.3,-0.5) -- (n1_P0);
\end{scope}
\end{tikzpicture}

